Perception Prioritized Training of Diffusion Models

Diffusion models learn to restore noisy data, which is corrupted with different levels of noise, by optimizing the weighted sum of the corresponding loss terms, i.e., denoising score matching loss. In this paper, we show that restoring data corrupted with certain noise levels offers a proper pretext task for the model to learn rich visual concepts. We propose to prioritize such noise levels over other levels during training, by redesigning the weighting scheme of the objective function. We show that our simple redesign of the weighting scheme significantly improves the performance of diffusion models regardless of the datasets, architectures, and sampling strategies.

==> tables/rebuttal-fid.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|cc|cc}
\hline
         & \multicolumn{2}{c|}{FID$\downarrow$} & \multicolumn{2}{c}{KID$\downarrow$ ($\times 10^3$)} \\ \hline
Dataset  & Base      & Ours              & Base     & Ours               \\ \hline
FFHQ     &    9.33   &  \textbf{8.44}    &   3.86   &  \textbf{3.54}     \\
CUB      &    10.75  & \textbf{7.73}     &   3.67    & \textbf{2.41}      \\ 
AFHQ-D   & 13.03   &   \textbf{12.15}   &    4.81     &    \textbf{3.93}   \\ \hline

\end{tabular}
\vspace{-0.8em}
\caption{\textbf{Results with 1k sampling steps.} FID(10k) and KID(10k) are measured between 10k samples generated with 1k steps and all training images. Same models are used as Table 1 of the main text except AFHQ-Dog, where we retrained with dropout. %We used relatively light models (94M params) while previous works rely on heavier models ([8]-552M, [14]-114M).
}
\vspace{-1.5em}
\label{table:fid_rebuttal}
\end{table}
